Feasibility of first principles molecular dynamics in fault-tolerant quantum computer by quantum phase estimation

This article shows a proof of concept regarding the feasibility of ab initio molecular simulation, wherein the wavefunctions and the positions of nuclei are simultaneously determined by the quantum algorithm, as is realized by the so-called Car-Parrinello method by classical computing. The approach used in this article is of a hybrid style, which shall be realized by future fault-tolerant quantum computer. First, the basic equations are approximated by polynomials. Second, those polynomials are transformed to a specific form, wherein all variables (representing the wavefunctions and the atomic coordinates) are given by the transformations acting on a linear space of monomials with finite dimension, and the unknown variables could be determined as the eigenvalues of those transformation matrices. Third, the eigenvalues are determined by quantum phase estimation. Following these three steps, namely, symbolic, numeric, and quantum steps, we can determine the optimized electronic and atomic structures of molecules.

==> matricesdata.tex <==
\section{Matirx data used in the article}

In the following, the data of $m_x$, and $m_r$, and $m_e$ are shown by a kind of heat-maps. The entry $A_{ij}$ in the matrix are indicated by 0 or 1 if it is  equal to either of those values; unless it is given by the symbol X. 

\begin{verbatim}    
mx:=
||000000X0X0XXX0X0XX0XXX||
||000000X0X0XXX0X0XX0XXX||
||000000X0X0XXX0X0XX0XXX||
||000000X0X0XXX0X0XX0XXX||
||000000X0X0XXX0X0XX0XXX||
||000000X0X0XXX0X0XX0XXX||
||1000000000000000000000||
||000000X0X0XXX0X0XX0XXX||
||0100000000000000000000||
||000000X0X0XXX0X0XX0XXX||
||0010000000000000000000||
||0001000000000000000000||
||0000100000000000000000||
||000000X0X0XXX0X0XX0XXX||
||0000010000000000000000||
||0000001000000000000000||
||0000000100000000000000||
||0000000001000000000000||
||0000000000001000000000||
||0000000000000100000000||
||0000000000000001000000||
||0000000000000000001000||
max= 258.60441684588295 min= -72.19094270794328

mr:=
||XXXXXX0X0X000X0X00X000||
||XXXXXX0X0X000X0X00X000||
||XXXXXX0X0X000X0X00X000||
||XXXXXX0X0X000X0X00X000||
||1000000000000000000000||
||0100000000000000000000||
||000000X0X0XXX0X0XX0XXX||
||0010000000000000000000||
||000000X0X0XXX0X0XX0XXX||
||0001000000000000000000||
||000000X0X0XXX0X0XX0XXX||
||000000X0X0XXX0X0XX0XXX||
||0000001000000000000000||
||0000000100000000000000||
||0000000010000000000000||
||0000000001000000000000||
||0000000000100000000000||
||0000000000010000000000||
||0000000000000001000000||
||0000000000000000100000||
||0000000000000000010000||
||0000000000000000000010||
max= 3484.3400839743654 min= -608.2044403624424

me:=
||XXXXXX0X0X000X0X00X000||
||XXXXXX0X0X000X0X00X000||
||XXXXXX0X0X000X0X00X000||
||XXXXXX0X0X000X0X00X000||
||XXXXXX0X0X000X0X00X000||
||XXXXXX0X0X000X0X00X000||
||000000X0X0XXX0X0XX0XXX||
||0100000000000000000000||
||000000X0X0XXX0X0XX0XXX||
||0010000000000000000000||
||000000X0X0XXX0X0XX0XXX||
||000000X0X0XXX0X0XX0XXX||
||000000X0X0XXX0X0XX0XXX||
||0000010000000000000000||
||000000X0X0XXX0X0XX0XXX||
||0000000100000000000000||
||0000000010000000000000||
||0000000000100000000000||
||0000000000000100000000||
||0000000000000010000000||
||0000000000000000100000||
||0000000000000000000100||
max= 4115.255552663199 min= -1486.152450941102
\end{verbatim}

\begin{landscape}
mx
$$
\begin{array}{cccccccccccccccccccccc}
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.75 &  0.00 &  0.02 &  0.00 & -0.03 & -0.00 & -2.90 &  0.00 &  0.10 &  0.00 & -0.06 &  0.02 &  0.00 &  0.60 & -0.24 &  0.95\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  10.66 &  0.00 &  0.41 &  0.00 & -0.15 & -0.26 & -72.19 &  0.00 &  1.90 &  0.00 & -2.20 &  1.25 &  0.00 &  9.85 & -3.76 &  15.94\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -41.69 &  0.00 & -1.75 &  0.00 &  0.56 &  0.91 &  258.60 &  0.00 & -7.74 &  0.00 &  3.96 & -4.87 &  0.00 & -28.11 &  12.11 & -49.34\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  22.54 &  0.00 & -0.50 &  0.00 &  0.23 &  0.07 & -47.51 &  0.00 & -2.39 &  0.00 &  1.06 &  0.48 &  0.00 & -8.99 & -2.07 &  0.89\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.05 &  0.00 &  0.00 &  0.00 & -0.00 & -0.00 & -0.04 &  0.00 &  0.01 &  0.00 & -0.01 &  0.00 &  0.00 &  0.06 & -0.04 &  0.08\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -2.01 &  0.00 & -0.10 &  0.00 &  0.01 &  0.03 &  12.49 &  0.00 & -0.45 &  0.00 &  0.38 & -0.22 &  0.00 & -2.75 &  1.06 & -4.13\\
  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -13.29 &  0.00 & -0.56 &  0.00 &  0.21 &  0.29 &  83.40 &  0.00 & -2.47 &  0.00 &  1.28 & -1.36 &  0.00 & -9.55 &  3.25 & -16.11\\
  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  2.96 &  0.00 & -0.16 &  0.00 &  0.07 &  0.02 &  8.88 &  0.00 & -0.76 &  0.00 &  0.33 &  0.15 &  0.00 & -2.85 & -0.66 & -2.16\\
  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -2.58 &  0.00 & -0.11 &  0.00 &  0.05 &  0.06 &  16.39 &  0.00 & -0.49 &  0.00 &  0.24 & -0.29 &  0.00 & -1.88 &  0.66 & -3.30\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00
\end{array}
$$
\end{landscape}
me
$$
\begin{array}{ c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c}
  2.96 & -0.16 &  0.07 &  0.02 &  8.88 & -0.76 &  0.00 &  0.33 &  0.00 &  0.15 &  0.00 &  0.00 &  0.00 & -2.85 &  0.00 & -0.66 &  0.00 &  0.00 & -2.16 &  0.00 &  0.00 &  0.00\\
 -232.95 & -12.87 &  7.06 &  5.21 &  1727.54 & -37.47 &  0.00 &  5.05 &  0.00 & -20.64 &  0.00 &  0.00 &  0.00 & -177.45 &  0.00 &  41.82 &  0.00 &  0.00 & -334.09 &  0.00 &  0.00 &  0.00\\
 -259.53 & -11.06 &  8.21 &  4.17 &  1630.81 & -52.88 &  0.00 &  36.51 &  0.00 & -20.66 &  0.00 &  0.00 &  0.00 & -274.32 &  0.00 &  92.81 &  0.00 &  0.00 & -433.28 &  0.00 &  0.00 &  0.00\\
 -562.07 & -21.85 &  8.69 &  15.98 &  3484.34 & -96.30 &  0.00 &  45.62 &  0.00 & -46.30 &  0.00 &  0.00 &  0.00 & -375.98 &  0.00 &  82.27 &  0.00 &  0.00 & -608.20 &  0.00 &  0.00 &  0.00\\
  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  2.96 &  0.00 & -0.16 &  0.00 &  0.07 &  0.02 &  8.88 &  0.00 & -0.76 &  0.00 &  0.33 &  0.15 &  0.00 & -2.85 & -0.66 & -2.16\\
  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -232.95 &  0.00 & -12.87 &  0.00 &  7.06 &  5.21 &  1727.54 &  0.00 & -37.47 &  0.00 &  5.05 & -20.64 &  0.00 & -177.45 &  41.82 & -334.09\\
  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -259.53 &  0.00 & -11.06 &  0.00 &  8.21 &  4.17 &  1630.81 &  0.00 & -52.88 &  0.00 &  36.51 & -20.66 &  0.00 & -274.32 &  92.81 & -433.28\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -562.07 &  0.00 & -21.85 &  0.00 &  8.69 &  15.98 &  3484.34 &  0.00 & -96.30 &  0.00 &  45.62 & -46.30 &  0.00 & -375.98 &  82.27 & -608.20\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00
\end{array}
$$
mr
$$
\begin{array}{ c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c, c}
 -13.29 & -0.56 &  0.21 &  0.29 &  83.40 & -2.47 &  0.00 &  1.28 &  0.00 & -1.36 &  0.00 &  0.00 &  0.00 & -9.55 &  0.00 &  3.25 &  0.00 &  0.00 & -16.11 &  0.00 &  0.00 &  0.00\\
 -662.55 & -21.38 & -12.61 &  16.52 &  4115.26 & -167.19 &  0.00 &  259.82 &  0.00 & -115.60 &  0.00 &  0.00 &  0.00 & -1006.95 &  0.00 &  495.12 &  0.00 &  0.00 & -1486.15 &  0.00 &  0.00 &  0.00\\
 -232.95 & -12.87 &  7.06 &  5.21 &  1727.54 & -37.47 &  0.00 &  5.05 &  0.00 & -20.64 &  0.00 &  0.00 &  0.00 & -177.45 &  0.00 &  41.82 &  0.00 &  0.00 & -334.09 &  0.00 &  0.00 &  0.00\\
 -259.53 & -11.06 &  8.21 &  4.17 &  1630.81 & -52.88 &  0.00 &  36.51 &  0.00 & -20.66 &  0.00 &  0.00 &  0.00 & -274.32 &  0.00 &  92.81 &  0.00 &  0.00 & -433.28 &  0.00 &  0.00 &  0.00\\
 -2.58 & -0.11 &  0.05 &  0.06 &  16.39 & -0.49 &  0.00 &  0.24 &  0.00 & -0.29 &  0.00 &  0.00 &  0.00 & -1.88 &  0.00 &  0.66 &  0.00 &  0.00 & -3.30 &  0.00 &  0.00 &  0.00\\
  81.09 &  2.16 &  4.36 & -2.14 & -468.59 &  20.77 &  0.00 & -50.96 &  0.00 &  19.34 &  0.00 &  0.00 &  0.00 &  160.04 &  0.00 & -92.23 &  0.00 &  0.00 &  229.03 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -13.29 &  0.00 & -0.56 &  0.00 &  0.21 &  0.29 &  83.40 &  0.00 & -2.47 &  0.00 &  1.28 & -1.36 &  0.00 & -9.55 &  3.25 & -16.11\\
  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -662.55 &  0.00 & -21.38 &  0.00 & -12.61 &  16.52 &  4115.26 &  0.00 & -167.19 &  0.00 &  259.82 & -115.60 &  0.00 & -1006.95 &  495.12 & -1486.15\\
  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -232.95 &  0.00 & -12.87 &  0.00 &  7.06 &  5.21 &  1727.54 &  0.00 & -37.47 &  0.00 &  5.05 & -20.64 &  0.00 & -177.45 &  41.82 & -334.09\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -259.53 &  0.00 & -11.06 &  0.00 &  8.21 &  4.17 &  1630.81 &  0.00 & -52.88 &  0.00 &  36.51 & -20.66 &  0.00 & -274.32 &  92.81 & -433.28\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 & -2.58 &  0.00 & -0.11 &  0.00 &  0.05 &  0.06 &  16.39 &  0.00 & -0.49 &  0.00 &  0.24 & -0.29 &  0.00 & -1.88 &  0.66 & -3.30\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  81.09 &  0.00 &  2.16 &  0.00 &  4.36 & -2.14 & -468.59 &  0.00 &  20.77 &  0.00 & -50.96 &  19.34 &  0.00 &  160.04 & -92.23 &  229.03\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00\\
  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  1.00 &  0.00 &  0.00
\end{array}
$$
